Neur2BiLO: Neural Bilevel Optimization

Bilevel optimization deals with nested problems in which a leader takes the first decision to minimize their objective function while accounting for a follower's best-response reaction. Constrained bilevel problems with integer variables are particularly notorious for their hardness. While exact solvers have been proposed for mixed-integer linear bilevel optimization, they tend to scale poorly with problem size and are hard to generalize to the non-linear case. On the other hand, problem-specific algorithms (exact and heuristic) are limited in scope. Under a data-driven setting in which similar instances of a bilevel problem are solved routinely, our proposed framework, Neur2BiLO, embeds a neural network approximation of the leader's or follower's value function, trained via supervised regression, into an easy-to-solve mixed-integer program. Neur2BiLO serves as a heuristic that produces high-quality solutions extremely fast for four applications with linear and non-linear objectives and pure and mixed-integer variables.

==> definitions.tex <==
% Sets
% \newcommand{\xofi}{x^i}
% \newcommand{\xminusi}{x^{-i}}
% \newcommand{\X}[1]{ \mathcal{X}^{ #1 } } 
% \newcommand{\ones}{\mathbf 1}
% \newcommand{\Z}{\mbox{\bf Z}}
% \newcommand{\Sy}{\mbox{\bf S}} 
% \newcommand{\NPhard}{\mbox{$\mathcal{NP}$-hard}}  
% \newcommand{\SigmaTwoP}{\mbox{$\Sigma^p_2$-hard}} 
% \newcommand{\prob}{ {\mathbf P} }
% \newcommand{\identity}{I}
% \newcommand{\nullspace}{ {\mathcal N} }
% \newcommand{\range}{ {\mathcal R} }
% \newcommand{\Rank}{\operatorname{\bf Rank}}
% \newcommand{\diag}{\operatorname{\bf diag}}
% \newcommand{\lambdamax}{\lambda_{\rm max} } 
% \newcommand{\lambdamin}{\lambda_{\rm min}}
% \newcommand{\Expect}{\operatorname{\bf E{}}}
% \newcommand{\Prob}{\operatorname{\bf Prob}}
% \newcommand{\dist}{\operatorname{\bf dist{}}}
% \newcommand{\sol}{\operatorname{SOL}}
% \newcommand{\conv}{\operatorname{conv}}
% \newcommand{\intr}{\operatorname{int}}
% \newcommand{\relintr}{\operatorname{relint}}
% \newcommand{\relint}{\relintr}
% \newcommand{\rec}{\operatorname{rec}}
% \newcommand{\lin}{\operatorname{lin}}
% \newcommand{\bd}{\operatorname{bd}}
% \newcommand{\cl}{\operatorname{cl}}
% \newcommand{\proj}{\operatorname{proj}}
% \newcommand{\sgn}{\operatorname{sgn}}
% \newcommand{\cone}{\operatorname{cone}}
% \newcommand{\epi}{\operatorname{\bf epi}} % epigraph
% \newcommand{\Vol}{\operatorname{\bf vol}}
% \newcommand{\dom}{\operatorname{\bf dom}} % domain

% \newcommand{\sign}{\operatorname{\bf sign}}
% \newcommand{\round}{\operatorname{\bf round}}
% \newcommand{\define}{\coloneqq}

% Trees
\newcommand{\tree}{\mathcal{T}}

% Strategy
\newcommand{\strategy}{\mathcal{S}}
\newcommand{\intvars}{\mathcal{I}}
\newcommand{\tightconstraints}{\mathcal{T}}

% Machine learning
\newcommand{\loss}{\mathcal{L}}

% Sections (for citation)
\newcommand{\Sec}{Section\;}

% Create theorems and other environments
%\newtheorem{theorem}{Theorem} % Restart counter every section
\newtheorem{lemma}{Lemma}  % Restart counter every section
% \newtheorem{corollary}{Corollary}[theorem]  % Restart counter every theorem
\newtheorem{proposition}{Proposition}%[section]
% \newtheorem{assumption}{Assumption}[section]
% \newtheorem{definition}{Definition}[section]
% \newtheorem{example}{Example}[section]
% \newtheorem{exercise}{Exercise}[section]
% \newtheorem{remark}{Remark}[section]
% \newtheorem{problem}{Problem}[section]


% Add Clevref names
\newtheorem{observation}{Observation}  % Restart counter every section
\crefname{line}{Line}{Lines}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{observation}{Observation}{Observations}
\crefname{equation}{}{}
\crefname{definition}{Definition}{Definitions}
\crefname{claim}{Claim}{Claim}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{remark}{Remark}{Remarks}
\crefname{example}{Example}{Examples}
\crefname{figure}{Figure}{Figures}
\crefname{section}{Section}{Sections}
\crefname{table}{Table}{Tables}

\newcommand{\method}{\textsc{Neur2BiLO}}

\newcommand{\mls}{NN$^l$}
\newcommand{\mlu}{NN$^u$}
\newcommand{\mld}{NN$^d$}
\newcommand{\mln}{NN$^n$}

\newcommand{\gbts}{GBT$^l$}
\newcommand{\gbtu}{GBT$^u$}

\newcommand{\solver}{B\&C}
\newcommand{\greedy}{G-VFA}
\newcommand{\drbaseline}{B\&C+}
\newcommand{\mkkt}{MKKT}



==> head.tex <==
% Images and plots
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{graphicx, pgfplots, subfigure, standalone, pgf, tikz}
\usepackage[inline]{enumitem}
\usepackage[justification=justified,singlelinecheck=false]{caption}

%Biblio
\usepackage[sort&compress,numbers]{natbib}

% Utilities
\usepackage{comment, url,float, setspace, xspace}
%\pgfplotsset{compat=1.18} 

% Math
\usepackage{amsmath, amssymb, amsthm, amsfonts, mathtools, array, bm, xfrac}
\renewcommand{\qedsymbol}{$\blacksquare$}
\renewcommand\arraystretch{1.2}
\setlist[enumerate]{label=(\roman*.)}

% Algorithms
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}

% Definition of Optimization problems
\usepackage[short,c2,nocomma]{optidef}

% Hyperreferences
\usepackage[colorlinks,
            linkcolor=BlueViolet,
            citecolor=blue,
            urlcolor=blue]{hyperref}

% References to objects
\usepackage[nameinlink]{cleveref}

% Tables
\usepackage{csvsimple, booktabs, longtable, multirow, multicol, adjustbox}	% reading CSV files in tables

% Acronyms
\usepackage[xindy, acronyms, nowarn]{glossaries}   % Glossaries and Acronyms
\makeglossaries

% Todos
\newcommand{\todo}[1]{{\color{Turquoise} \texttt{\#TODO }#1}}


%ORCIDs
\definecolor{lime}{HTML}{A6CE39}
\DeclareRobustCommand{\orcidicon}{
	\begin{tikzpicture} \draw[lime, fill=lime] (0,0) circle [radius=0.16] node[white] { {\fontfamily{qag}\selectfont \tiny ID} };
	\draw[white, fill=white] (-0.0625,0.095) circle [radius=0.007];
	\end{tikzpicture} \hspace{-2mm}
}

\foreach \x in {A, ..., Z}{\expandafter\xdef\csname orcid\x\endcsname{\noexpand\href{https://orcid.org/\csname orcidauthor\x\endcsname}{\noexpand\orcidicon} } }
% Bibliography
\bibliographystyle{plainnat}


